LLMTreeRec: Unleashing the Power of Large Language Models for Cold-Start Recommendations

The lack of training data gives rise to the system cold-start problem in recommendation systems, making them struggle to provide effective recommendations. To address this problem, Large Language Models (LLMs) can model recommendation tasks as language analysis tasks and provide zero-shot results based on their vast open-world knowledge. However, the large scale of the item corpus poses a challenge to LLMs, leading to substantial token consumption that makes it impractical to deploy in real-world recommendation systems. To tackle this challenge, we introduce a tree-based LLM recommendation framework LLMTreeRec, which structures all items into an item tree to improve the efficiency of LLM's item retrieval. LLMTreeRec achieves state-of-the-art performance under the system cold-start setting in two widely used datasets, which is even competitive with conventional deep recommendation systems that use substantial training data. Furthermore, LLMTreeRec outperforms the baseline model in A/B testing on Huawei industrial systems. Consequently, LLMTreeRec demonstrates its effectiveness as an industry-friendly solution that has been successfully deployed online. Our code is available at: https://github.com/Applied-Machine-Learning-Lab/LLMTreeRec.

==> 7Limitations.tex <==
\section{Limitations}
Our proposed UniLLMRec can effectively work on large-scale item corpus in a zero-shot manner.
It mainly leverages the semantic item tree, by dynamically updating its structure in real-time.
Therefore, there is no need for LLM fine-tuning to cater dynamic item updates. 
Nevertheless, the tree is manually constructed based on item semantic information, similar items with subtle semantic differences can be assigned to different subcategories, thus introducing noises to our model. 
% On one hand, the manually created item tree may suffer from inaccuracy in semantic information. 
Additionally, issues such as structural imbalance and uneven item set sizes in leaf nodes exist in the constructed item tree. 
For instance, in the MIND dataset, a majority of news concentrates on a few subcategories.
Similar issues arise in the Amazon dataset, exhibiting the imbalanced distribution of the constructed tree. 
We leave it for future work to construct a balanced item tree with accurate semantic information.

% \section*{Ethics Statement}
% The proposed LLM-centered recommendation systems leverage user interaction history to infer user interests and conduct recommendation tasks. Therefore, on the one hand, for privacy concerns, the utilization of user data for inference is contingent upon obtaining explicit user consent. On the other hand, though concerns regarding fairness in large language models may arise, our proposed model solely relies on user historical interaction data, avoiding any involvement with sensitive user attributes, thus mitigating potential fairness issues associated with these features.

==> cover_letter.tex <==
\newcommand{\coverletter}{
    \clearpage 
    \null
    \vfill
    \begin{center}
        \Huge \textbf{Cover Letter}
    \end{center}
    \vspace*{2.5ex}
    
    \begin{flushright}
        February 01, 2024
        
        Wenlin Zhang, Chuhan Wu, Xiangyang Li, Yuhao Wang
        
        Kuicai Dong, Yichao Wang, Xinyi Dai, Xiangyu Zhao
        
        Huifeng Guo, Ruiming Tang
        \vspace*{2.5ex}
    \end{flushright}

    \begin{flushleft}
    ACM Transactions on Information Systems
    
    Dear Editors and Reviewers,
    \vspace*{2.5ex}
    \end{flushleft}

Thanks for considering our submission "Tired of Plugins? Large Language Models Can Be End-To-End Recommenders". To respond to the concerns of this journal, we list our statements for this submission.
\vspace*{2.5ex}

Here are our statements for submission:

\begin{enumerate}
    \item We confirm that the paper is not currently under submission at another journal or conference.
    \item There are no any our previous publications that significantly overlap with the submission.
    \item We confirm that all authors are aware of the submission and agree to its review by TOIS. 
    \item Our suggestions of three Associate Editors that seem most suitable to handle the submission are: Zi Huang, Grace Hui Yang, and Yongfeng Zhang.
    \item We confirm that there is no COI with the EiC and any AE.
    \item We confirm that our coverage of related work is appropriate and up-to-date. 
\end{enumerate}
% 1. We confirm that the paper is not currently under submission at another journal or conference. 

% 2. There are no any our previous publications that significantly overlap with the submission.

% 3. We confirm that all authors are aware of the submission and agree to its review by TOIS. 

% 4. Our suggestions of three Associate Editors that seem most suitable to handle the submission are: Zi Huang, Grace Hui Yang, and Yongfeng Zhang.

% 5. We confirm that there is no COI with the EiC and any AE.

% 6. We confirm that our coverage of related work is appropriate and up-to-date. 
\vspace*{2.5ex}

Your reviews and consideration of our article for publishing at ACM Transactions on Information Systems are greatly appreciated.
\vspace*{2.5ex}

Sincerely,

Wenlin Zhang, Chuhan Wu, Xiangyang Li, Yuhao Wang, Kuicai Dong, Yichao Wang, Xinyi Dai, Xiangyu Zhao, Huifeng Guo, Ruiming Tang

    \vfill 
    \null
    \newpage
}
